Accelerating Time Series Analysis via Processing using Non-Volatile Memories

Time Series Analysis (TSA) is a critical workload to extract valuable information from collections of sequential data, e.g., detecting anomalies in electrocardiograms. Subsequence Dynamic Time Warping (sDTW) is the state-of-the-art algorithm for high-accuracy TSA. We find that the performance and energy efficiency of sDTW on conventional CPU and GPU platforms are heavily burdened by the latency and energy overheads of data movement between the compute and the memory units. sDTW exhibits low arithmetic intensity and low data reuse on conventional platforms, stemming from poor amortization of the data movement overheads. To improve the performance and energy efficiency of the sDTW algorithm, we propose MATSA, the first Magnetoresistive RAM (MRAM)-based Accelerator for TSA. MATSA leverages Processing-Using-Memory (PUM) based on MRAM crossbars to minimize data movement overheads and exploit parallelism in sDTW. MATSA improves performance by 7.35x/6.15x/6.31x and energy efficiency by 11.29x/4.21x/2.65x over server-class CPU, GPU, and Processing-Near-Memory platforms, respectively.

==> sections/03-Motivation.tex <==
\section{Motivation}

In this section we present \myName{}'s motivation. Our proposal is motivated by 1) the wide applicability of time series analysis in a wide range of application domains and 2) sDTW's high data movement overheads in conventional architectures. 

\subsection{TSA Applications}

%Time series analysis is emerging as one of the most important data mining primitives for a wide variety of applications due its generality to detect anomalies and similarities. We present applications of TSA in Table~\ref{tab:tsa_applications}.
Time series analysis constitutes one of the most important data mining primitives thanks to its generality in detecting anomalies and similarities for a wide range of applications. Table~\ref{tab:tsa_applications} presents a few examples for applications of TSA.


\begin{table}[h!]
\centering
\resizebox{\linewidth}{!}{\begin{tabular}{|l|c||l|c|}
\hline
    \textbf{Field} & \textbf{References} & \textbf{Field} & \textbf{References}\\
\hline\hline
    Bioinformatics     &  \cite{brown2012adict, straume2004dna, bar2004analyzing} & Speech Recognition  &  \cite{balasubramanian2016discovering}\\
\hline
     Robotics          &  \cite{TIU05,Vahdatpour2009toward} & Weather Prediction &  \cite{McGovern2011identifying}\\
\hline
     Neuroscience & \cite{brown2012adict,Kolb1821evidence} & Entomology & \cite{Szigeti2015searching}\\
\hline
     Machine Learning & \cite{WarrenLiao2005clustering,Aghabozorgi2015time,KK03} & Geophysics & \cite{trugman2017growclust,Waldhauser2000adouble,Christophersen2018bayesian,McKee2018instrumental}\\
\hline
    Econometrics & \cite{Howrey1980therole} & Statistics & \cite{Shymway1988applied}\\
\hline
    Finance & \cite{Tsay2005analysis,nakagawa2019stock} & Control Engineering & \cite{George2009time, nelson1998two, barber2011bayesian}\\
\hline
    Signal Processing & \cite{Kumar2012time} & Pattern Recognition & \cite{berlin1994pattern}\\
\hline
    Communication & \cite{lakhina2004characterization, jain1986packet, barford2001characteristics} & Medicine & \cite{Hussain2017symbolic,Balli2008eeg, dunn2021squigglefilter,chen2020anomaly}\\
\hline
    Astronomy & \cite{Vio2004timeseries,Scargle1998studies} & Social Networks & \cite{nusratullah2015detecting, asur2010predicting}\\
\hline
    Clustering & \cite{WarrenLiao2005clustering,Aghabozorgi2015time} & Classification & \cite{KK03}\\
\hline
    Earthquakes & \cite{trugman2017growclust,Waldhauser2000adouble,Christophersen2018bayesian,McKee2018instrumental} & GPS Tracking & \cite{klos2018detecting}\\
\hline
    Virtual Reality & \cite{stoermer2000monitoring} & Gesture Recognition & \cite{hussain2012user,calin2016gesture}\\
\hline
    Trajectories & \cite{ayhan2016time} & Traffic Monitoring & \cite{li2015trend}\\
\hline
\end{tabular}}
\caption{Time Series Analysis main applications}
\label{tab:tsa_applications}
\vspace{-2mm}
\end{table}

In %the context of
statistics, econometrics, meteorology, and geophysics, the primary goal of time series analysis is prediction and forecasting. At the same time, in %the context of 
signal processing, control engineering, and communication engineering, it is used for signal detection and estimation. In data mining, pattern recognition, and machine learning, time series motif and discord discovery are used for clustering, classification, anomaly detection, and forecasting. Finally, the most important application of time series motif and discord discovery is clustering seismic data and discovering earthquake pattern clusters from the continuous seismic recording. Consequently, seismic clustering can be applied to earthquake relocation and volcano monitoring to help improve earthquake and volcanic hazard assessments.

\textbf{End-to-End Application Benefits of using TSA.} Accelerating TSA is critical for real-life examples of end-to-end applications. For instance, \cite{hyland2020early} predicts circulatory failure in intensive care units. In this scenario, 90\% of the execution time is dominated by TSA preprocessing, while the remainder 10\% is used by the machine learning-based application to perform the classification. We also find many other real use case examples that can benefit from this approach, such as:



\begin{itemize}
    \item \textbf{Earthquake detection}~\cite{Christophersen2018bayesian}. TSA can process the data from a seismograph and detect anomalies that can be further processed with complex algorithms.
    
    \item \textbf{Electroencephalography}~\cite{chen2020anomaly}. Assuming an electroencephalograph that is monitoring a patient, TSA can be used to detect anomalies and trigger an alarm about that.
    
    \item \textbf{Virus Detection}~\cite{dunn2021squigglefilter}. During the genome assembly process, basecalling is a compute-intensive task that can be skipped for most queries using a TSA-based filter.
\end{itemize}



%We conclude that time series motif and discord discovery are critical for many applications. Thus it is of vital importance to accelerate time series motif and discord discovery.
%in this work we aim to accelerate time series motif and discord discovering by proposing a specific architecture for general time series analysis.

\subsection{sDTW Bottlenecks}
\label{sec:bottlenecks}

We perform a detailed characterization of \di{parallel versions of} sDTW on different commodity computing systems.

\textbf{CPU platforms}. We profile the performance of sDTW using a manycore processor (Intel Xeon Phi 7210), analyzing the execution of 16K queries of 8K elements each that are compared against a reference sequence of 32K elements. Figure~\ref{fig:sdtw_roofline} presents the roofline plot for the experiment.
%such configuration.

\begin{figure}[h!]
    \centering
    \includegraphics[width=\linewidth]{figures/roofline.pdf}
    \caption{sDTW's roofline in an Intel Xeon Phi (64 cores, DDR4). The application is located in the memory-bound zone.}
    \label{fig:sdtw_roofline}
    \vspace{-2mm}
\end{figure}

First, we observe that sDTW only exploits 41\% of the system's integer peak performance, i.e., 59 GINTOPS out of 145 GINTOPS, and it presents low arithmetic intensity (0.55 INTOP/Byte). Second, we find that the memory footprint of the execution is $\approx$570MB. The total memory traffic generated during runtime is $\approx$267 GB, putting the kernel above the DDR4 peak bandwidth most of the execution time. \di{This means that sDTW, while highly parallelizable due to independence across queries, is memory-bound in manycore CPUs.} 


\textbf{GPU platforms}. We find that several prior works~\cite{zhu2018developing, liu2019high, chang2012efficient, coelho2017gpu, eslami2018fast} propose to accelerate sDTW using GPUs. However, these works rely on shared-memory optimizations that only perform for certain small query sizes. For large query sizes, these implementations either 1) do not work or 2) use high-latency global-memory to hold the main data structures of sDTW, which results in large performance penalties. We develop a CUDA-based implementation that supports arbitrary sizes.

\textbf{FPGA platforms}. Several prior works propose~\cite{kalantar2021fa, kang2020fpga, alomar2016fpga} to accelerate sDTW using FPGAs. However, most of them have very limited onboard memory, and data has to be moved over narrow buses. We develop our own HLS-based FPGA implementation and find that 1) the number of computation units is not enough to exploit the inherent parallelism of sDTW, and 2) the compute units spend most of their time waiting for the memory accesses to be served.%\cgiannou{again -it would be good to show evaluation plot/data to quantitatively prove this statement.}


\textbf{PNM/PuM platforms}. One way of improving parallelism and reducing data movement costs is to perform computation near or using memory. We analyze several approaches in those directions and detail their benefits and drawbacks.
\begin{itemize}
    \item \underline{\textit{General-purpose PNM}}. This approach typically places small CPU cores in the same die as DRAM. The main benefit of this scheme is that the architecture can be potentially used for general-purpose applications. However, this comes at the cost of limited parallelism. We evaluate a general-purpose PNM (\texttt{upmem} baseline) in \cref{sec:matsa_comparison}, and our evaluations show that this architecture is compute bound when performing the sDTW computation.
    % \christina{this is a bit contradicting, because the reader hasn't understand how close are the CPU to DRAM, and why the data movement is such a problem in that case... } \christina{I would remove the last sentence and I would write '? or it is still bottlenecked by data movement?}
    
    \item \underline{\textit{Specialized PNM}}. This approach typically places an ASIC accelerator in the same die as DRAM. The main benefit of this approach is that the processing elements are highly optimized for the target workload. However, the data still needs to be moved from memory to the accelerator. Even though an ASIC accelerator can be used in a PNM architecture, performance would still be bottlenecked by data movement between memory and the accelerator, similarly to general-purpose PNM.
    % \christina{We can write 'even though a ASIC accelerator can be used in a PNM architecture, performance would be still bottlenecked by data movement between memory and the accelator, similarly to General PNM (previsou item). }
    
    \item \underline{\textit{SRAM-based PuM}}. This approach uses SRAM-based memory arrays to perform in-situ computation (e.g., compute caches~\cite{aga2017compute}). The main benefits of this approach are the high levels of parallelism and reduced data movement. Unfortunately, SRAM suffers from density and scalability issues~\cite{gupta2019exploring}, along with being radiation vulnerable.
    
    \item \underline{\textit{DRAM-based PuM}}. This approach uses DRAM-based memory arrays to perform in-situ computation (e.g., SIMDRAM~\cite{hajinazar2021simdram}). However, this approach involves internal data movement to perform the operations, as data needs to be moved to specific compute-enabled rows before performing the actual operations. Moreover, DRAM suffers from data volatility and destructive read problems. %\christina{I insist that this sub-section would be benefit a lot by the figure that I mentioned some time ago.. qualitatively showing the data movement across the various architectures... We need to include this figure for the next submission}
    
\end{itemize}


\subsection{Need for an NVM-PuM TSA Accelerator}
TSA is widely applicable to many domains~\cite{WarrenLiao2005clustering}, while there is \emph{no} previous work to propose a 1) high performance, 2) energy-efficient, and 3) general solution. NVM-PuM architectures are promising candidates to match the requirements. %We conclude justifying the need for a NVM-based PuM TSA accelerator since 1) TSA is widely applicable to many domains and 2) there is no previous proposal that satisfy the requirements of TSA to enable an efficient solution.\cgiannou{remove the last sentence}

In contrast to the aforementioned proposals, NVM-PuM architectures 1) enable huge parallelism, 2) eliminate data movement costs, 3) provide better scalability than its competitors thanks to different levels of parallelism, 5) are CMOS-compatible, and 6) overcome the data volatility problem. 
% \christina{without power= 'can significantly reduce energy consumption thanks to its non-volatile nature?} 
The main drawback of NVM technologies is the lack of a well-established evaluation methodology. To tackle this issue, we perform an extensive design space exploration study in our evaluation using different NVM technologies.  

%On top of those reasons \christina{which reasons?}, the main goal of this work is to study the potential benefits in terms of performance and energy of an accelerator based on magnetoresistive devices to perform time series analysis. \christina{do we need this paragraph? We already mentioned the goal of this work.}


